Traffic Count Data Analysis Using Mixtures of Kato--Jones Distributions

We discuss the modelling of traffic count data that show the variation of traffic volume within a day. For the modelling, we apply mixtures of Kato-Jones distributions in which each component is unimodal and affords a wide range of skewness and kurtosis. We consider two methods for parameter estimation, namely, a modified method of moments and the maximum likelihood method. These methods were seen to be useful for fitting the proposed mixtures to our data. As a result, the variation in traffic volume was classified into the morning and evening traffic whose distributions have different shapes, particularly different degrees of skewness and kurtosis.

==> files/1_Intro.tex <==
\section{Introduction}
Traffic flow volume is one of the most essential variables in \chris{the} transport engineering field.
Also, it is easy to observe by installing \chris{a} traffic counter and counting the number of vehicles \chris{passing} by at the observation site.
Many traffic counters exist along arterial roads in Japan and other countries, and the traffic flow data are accumulated day by day \citep{led08,ana13}.

\chris{These} data are mainly utilized in the following two manners.
The first is evaluating road performance, or throughput, i.e., the maximum number of vehicles the road can accommodate within a unit time \citep{edi63,hcm}.
For example, this value is represented in \chriss{units} of vehicles per hour.
Traffic congestion occurs if more vehicles than this value come to the road.
The second is the so-called ``traffic state estimation'', which \chris{comprises} three essential variables: the traffic flow rate, the average vehicle density, and the average vehicle speed.
Understanding the relationship among these three variables is quite important to predict traffic congestion that \chris{is} spread along \chris{the} road network \citep{mun03,wan05}.
Both of \chris{road performance and traffic state estimation} deal with the observed traffic flow volume as aggregated data such as 1- or 5-\chris{minute} flow \chris{volumes}, i.e., the number of vehicles \chris{that} pass by in such time intervals.
In addition, some studies use such data without aggregation, i.e., the raw timestamp of each vehicle's passing.
They also aim at analyzing congestion and modeling the time intervals \chris{between} successive vehicles \citep{che10,li17}.

Utilizing the data in such ways is reasonable regarding the purpose of installing the traffic counter.
Nonetheless, the raw data may have much potential to bring additional insights to transport engineering.
For example, if we model the probability distribution of \kotar{time of} \chris{vehicles} passing, we can interpolate missing values, which may be caused by the failure of counters.
\kotar{Predicting} the traffic volume \kotar{in the whole road section including} unobserved locations may also be possible \kotar{by combining our model with interpolation methods}.
Additionally, it is useful for the verification and validation of microscopic traffic simulations that deal \chris{with} each vehicle as an agent.
To the best of \chris{the} authors' knowledge, no study except one written in Korean \citep{na11} estimates the probability distribution of traffic volume.

In this study, considering such potential applications, we estimate the \chris{complex} distribution of the variation of traffic volume within an average weekday.
Traffic volume is generally determined by the dynamic system of the interaction between the supply side (\kotar{i.e., how many vehicles the road can accommodate}) and the demand side (i.e., how many drivers wish to use the road).
Due to this complexity, the distribution of traffic volume in a day is not expected to be unimodal or symmetric.
\kotann{Generally, the timestamp of each vehicle's passing does not follow \chris{a} Poisson process because of some bottlenecks such as traffic congestion and traffic \chris{lights} \citep{dag97}.}
Actually, it is empirically bimodal and asymmetric on weekdays (explained in detail in Section \ref{data}).
\kota{In addition, if we consider an average weekday, time is periodic and represented as points on \chris{a} circle.
Thus, the time axis is circular in that 0 a.m. and 12 p.m. represent the same time.}
This suggests \chris{that} we had better employ directional statistics.

Our study is the first attempt to use the raw data of \chris{a} traffic counter and employ \chris{a} mixture of \katot{the circular distributions of \citet{kat15}} to represent the distribution of traffic volume in an average weekday.
Also, we contribute \chris{a} method of parameter estimation for \chris{mixtures} of Kato--Jones \chris{distributions} as there is no established method thus far.
\katorr{The use of mixtures of \katot{the distributions of \citet{kat15}} has been briefly discussed for an analysis of another traffic \chris{dataset} in the conference proceedings of \citet{nag19}.
However, despite its simplicity, it is not \chris{the case} that their inferential algorithm for the mixtures guarantees the consistency or any other optimal property of the proposed estimator.}

\katot{Some mixtures of circular distributions have been proposed in the literature.}
The most attention \chris{has} been paid to mixtures of von Mises distributions \citep[e.g.,][]{wal00,moo03,ban05,mul20}.
The components of \chris{these} mixtures, the von Mises distributions, are symmetric distributions with two parameters controlling location and mean resultant length.
Recently, \citet{miy20} discussed mixtures of sine-skewed distributions whose components can adopt mildly asymmetric shapes.
However, none of these existing models seem to be appropriate for our traffic data because one of the clusters \chris{in} our data is strongly skewed.
Therefore, for the modelling of our data, it seems reasonable to consider the distributions of \citet{kat15} as possible components of the mixtures because \chris{these distributions} can control a wide range of skewness as well as kurtosis.

The paper is organized as follows.
\chris{The traffic} count data of interest are introduced in Section \ref{data}.
We define the mixtures of the distributions of \citet{kat15}, which are applied to the traffic data, and investigate basic properties of the mixtures and their components in Section \ref{sec:model}.
Two methods for parameter estimation for the proposed mixtures are presented in Section \ref{sec:estimation}.
A simulation study is conducted to compare the two proposed methods for parameter estimation in Section \ref{sec:simulation}.
The proposed mixtures are applied to the traffic data using the proposed inferential methods in Section \ref{sec:application}.
The interpretation of the estimated model is also discussed.
The fit of the proposed mixtures to the data is compared with the fits of some other mixture models in Section \ref{sec:comparison}.
Finally, Section \ref{sec:conclusion} concludes the paper.
The online Supplementary Materials provide the additional data analysis, a simulation study, proofs of the claims made in the main article, and Python codes for parameter estimation.
%proofs of Theorem 1 and Proposition 1 and Python codes for parameter estimation and simulation study.

==> files/2_Data.tex <==
\section{The Data}
\label{data}
First, we briefly explain about traffic counters in general.
Traffic counters record the timestamps of all \chris{vehicles} passing. 
Many counters are installed along the arterial roads in Japan, \chris{often} at intervals of one kilometer.
Usually, these data are aggregated to 1- or 5-\chris{minute} vehicle counts.
Then, the aggregated data are utilized for traffic control such as detecting congestion and providing information to drivers.
On the other hand, we use the data without aggregation in this paper, the data \chris{being} raw timestamps, to model the probability of \chris{a} vehicle passing at \chris{each particular time}.
In particular, this paper focuses on the averaged \chris{distribution for} weekdays.
Then, the time axis is circular; 0:00 (0 a.m.) and 24:00 (12 p.m.) represent the same time, and 1:00 (1 a.m.) and 23:00 (11 p.m.) are not 22 hours apart, but only 2 hours apart.
To consider \chris{these} characteristics accurately, we employ the concept of directional statistics.

\chris{Concretely}, we use the data of a traffic counter provided by \chris{the} Hanshin Expressway Co. Ltd., Japan \chris{via} personal communication.
Specifically, the data are obtained at \chris{the} 20.4 kilopost of \chris{the} Kobe route, Hanshin \katot{Expressway.
Fig.\ \ref{fig:target area} shows \chris{a} map of the target area including the location of the traffic counter and \chris{the} Kobe route of \chris{the} Hanshin Expressway.
\chris{The} background map is based on \chris{a} Digital Map by \chris{the} Geospatial Information Authority of Japan.}
\begin{figure}
\centering
\includegraphics[clip,keepaspectratio,width=0.7\textwidth]{fig/fig1.pdf}
\caption{\label{fig:target area} Map of target area \katot{including the location of the traffic counter and \chris{the} Kobe route of \chris{the} Hanshin Expressway}.}
\end{figure}
\katot{\chris{The} Kobe route} exists in \chris{the} Osaka metropolitan area and connects two large cities, Osaka and Kobe.
\chris{The} Osaka metropolitan area is the second largest megacity in Japan following \chris{the} Tokyo metropolis and its population is around 20 \chris{million}. 
Osaka city is the \chris{main} city of \chris{the} Osaka metropolitan area with \chris{a} population of around 2.8 \chris{million}.
Kobe city is the second largest city in the area with \chris{a} population of 1.5 \chris{million} and \chris{is} located about 30 km west of Osaka city.

The counter records the timestamps of \chris{vehicles} passing in the direction from Kobe to Osaka.
The data period is 46 weekdays; from June 6th to July 7th and from August 22nd to October 10th in 2016.
\kotan{\katot{It is not unnatural to aggregate data for all weekdays because the \chris{distribution} of weekday traffic is generally similar \citep{hcm}.}}
\chris{A} histogram of the data of the summation of all 46 days \chris{is} shown in Fig.\ \ref{fig:weekday}. 
The bin width is set as 1 hour for this figure.

\begin{figure}
\centering
\includegraphics[clip,keepaspectratio,width=0.75\textwidth]{./fig/weekday.pdf}
\caption{\label{fig:weekday} \chris{A} histogram of the data for the summation of all 46 weekdays.}
\end{figure}

The total number of observed vehicles for 46 days is 1,121,262, which equals 24,375 per day on average.
Here, the histogram has two peaks at around 7:00 and 15:00.
We assume that the former peak represents the morning rush hour and the latter does the evening rush hour, from Kobe to Osaka, as the data are for weekdays.
\kotar{Note that all recorded traffic is in the same direction (i.e., from Kobe to Osaka).
It means that vehicles commuting to their office and returning home are observed only once in the morning or evening.}

In addition, the peak in the morning is higher and sharper than that in the evening.
Also, each peak has \chris{an} asymmetric shape.
For example, as many commuters should arrive \chris{at} their \chris{offices} in Osaka at around the same \katot{time, typically, at 8:30 or 9:00,} the histogram of the morning peak suggests \chris{a} negatively-skewed shape.
\kotar{A model that cannot represent flexible shapes cannot adequately describe traffic data's shape and characteristics.}
To fully represent the characteristics of this distribution, a mixture of \katot{probability density functions} that allows a flexible shape is necessary.
\kotar{
Hereafter, we assume that the data follow the IID property.
Although this might be a strong assumption, it seems acceptable from the transportation engineering viewpoint.
See Appendix A of Supplementary Material for the details.
}

==> files/5_Simulation.tex <==
\katot{
\section{\kotan{Simulation study}} \label{sec:simulation}
}

We compare the performance of the modified method of moments estimation and the maximum likelihood estimation by EM algorithm via a Monte Carlo simulation study.
Random samples of sizes $n=50, 100, 500, 1000, $ and $5000$ were generated from the estimated distribution whose parameters are shown in Table \ref{tab:em} (b).
For each sample size, $r=2000$ samples were generated.

For comparison of the two estimators, we employ the generalized mean squared error which is defined by $\det{(\Sigma)}$, where $\Sigma=E\{(\hat{\xi}-\xi)(\hat{\xi}-\xi)^T\}$ and $\hat{\xi}$ is an estimator of \katot{$\xi=(\mu_1,\mu_2,\rho_1,\rho_2,\lambda_1,\lambda_2,\pi'_1,\pi'_2)^T$.}
An estimate of the generalized mean squared error is given by replacing $\Sigma$ by its sample analogue $\hat{\Sigma}=r^{-1}\sum^{r}_{j=1}{(\hat{\xi}_j-\xi)(\hat{\xi}_j-\xi)^T}$, where the $\hat{\xi}_j$'s\chris{,} $j=1,...,r$\chris{,} are the estimates from the $r$ simulation samples.
We \chris{also} consider the estimated relative generalized mean squared error of the estimate via the modified method of moments with respect to the maximum likelihood estimate, which is defined as
\begin{equation*}
	\widehat{\rm{RGMSE}}=\frac{\det{(\hat{\Sigma}_{MM}})}{\det{(\hat{\Sigma}_{ML}})}\chris{.}
	\label{eq:rgmse}
\end{equation*}
\chris{Here,} $\hat{\Sigma}_{MM}$ and $\hat{\Sigma}_{ML}$ are sample estimates of the mean squared error matrices of modified method of moments estimation and maximum likelihood estimation, respectively.

For numerical optimization of ETM, \chris{the} scipy.optimize.minimize package in Python with SLSQP method is employed \citep{jon01,kra88}.
This method is a kind of quasi-Newton method and enables us to solve the constrained optimization problem.
In this analysis, the optimization of ETM is terminated \chris{when} the difference \chris{in} the value of ETM between two successive steps is lower than $1\times10^{-10}$.
The initial values of $\mu_k$, $\rho_k$ and $\lambda_k$ are random samples from the uniform distribution on the intervals $[0,2\pi)$, $[0,1)$ and $[0,2\pi)$, respectively.
Also, those of $\pi_1'$, $\pi_2'$ and $\pi_3'$ are in $[0,1)$ and $\pi_1'+\pi_2'+\pi_3'=1$.
\kota{
For this sampling, two random values are drawn from the uniform distribution on $[0,1)$ and the smaller one is regarded as $r_1$ and the other as $r_2$.
Then, $\pi_1'=r_1$, $\pi_2'=r_2-r_1$, and $\pi_3'=1-r_2$ are calculated.}
Furthermore, the moment weight parameter $c$ in $w(p)$ is set to 0.9 because our experiments suggest that estimates with small $c$ are not stable with regard to fitting the data.

\kotar{100 estimates are obtained via this process, and the estimate whose value of ETM is smallest is set as the initial value for the maximum likelihood estimation.}
For numerical optimization \chris{in the} \katot{M-step, namely, Step 2 in Algorithm \ref{alg:em},} the same Python package as in the optimization of ETM is employed.
In this analysis, each M-step is terminated when the difference of the value of the objective function between two successive iterations is lower than $1\times10^{-6}$.
Also, \chris{the} whole EM algorithm is terminated when the difference of the log-likelihood function between two successive M-steps is lower than $n\times10^{-6}$.
In both estimates, it is assumed \chris{that} $\hat{\mu}_1<\hat{\mu}_2$.
%The conditions of the modified method of moments estimation \chris{are} the same \chriss{as} \chris{in} the previous section except for the number of initial values, which is set to 100 in this simulation.
%\chris{Maximum} likelihood estimation is achieved by the EM algorithm, whose initial value is the modified method of moments estimate and the threshold of termination for the EM algorithm is set to $n\times10^{-6}$.

\begin{table}
\caption{\label{tab:com} The values of $\det{(\hat{\Sigma}_{MM})}$, $\det{(\hat{\Sigma}_{ML})}$ and $\widehat{\rm{RGMSE}}$}
\centering
\fbox{
\begin{tabular}{c|ccccc}
$n$ & $n=50$ & $n=100$ & $n=500$ & $n=1000$ & $n=5000$ \\
\hline
$\det{(\hat{\Sigma}_{MM})}$ & $5.35\times10^{-9}$ & $7.00\times10^{-10}$ & $2.70\times10^{-13}$ & $4.25\times10^{-15}$ & $4.01\times10^{-20}$\\
$\det{(\hat{\Sigma}_{ML})}$ & $5.05\times10^{-8}$ & $6.41\times10^{-9}$ & $3.56\times10^{-12}$ & $1.33\times10^{-14}$ & $1.23\times10^{-22}$\\
$\widehat{\rm{RGMSE}}$ & 0.106 & 0.109 & 0.076 & 0.322 & 325.3\\
\end{tabular}}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[clip,keepaspectratio,width=0.75\textwidth]{fig/simu.pdf}
\caption{\label{fig:simu} \katoss{Plot of the value of $\det{(\hat{\Sigma}_{MM})}$ (bold) and $\det{(\hat{\Sigma}_{ML})}$ (dotted) in simulation study.}}
\end{figure}

Table \ref{tab:com} shows the value of $\det{(\hat{\Sigma}_{MM})}$, $\det{(\hat{\Sigma}_{ML})}$ and $\widehat{\rm{RGMSE}}$ for each sample size.
\kotar{In addition, Fig.\ \ref{fig:simu} shows the trend of the change of the value of $\det{(\hat{\Sigma}_{MM})}$ and $\det{(\hat{\Sigma}_{ML})}$ in different sample sizes.}
As the sample size $n$ increases, the value of $\det{(\hat{\Sigma}_{MM})}$ and $\det{(\hat{\Sigma}_{ML})}$ \chris{decreases}.
\kotar{The value of $\det{(\hat{\Sigma}_{MM})}$ at $n=50$ is smaller than $\det{(\hat{\Sigma}_{ML})}$, however, the value of $\det{(\hat{\Sigma}_{MM})}$ at $n=5000$ is larger than $\det{(\hat{\Sigma}_{ML})}$ because the degree of decline in value with respect to sample size is greater for $\det{(\hat{\Sigma}_{ML})}$ than for $\det{(\hat{\Sigma}_{MM})}$.
Therefore, the values of $\widehat{\rm{RGMSE}}$ are smaller than 1 for $n\leq1000$ and larger for $n=5000$.}
\kotar{These results imply} modified moments estimation is preferable for estimation from a small number of samples \kotar{in terms of $\widehat{\rm{RGMSE}}$}.
On the other hand, maximum likelihood estimation is preferable for estimation from a large number of samples such as the data in this paper.
Note that modified moments estimation \chris{yields} not only an estimate but also a good initial value \chris{for} maximum likelihood estimation.
Although the value of $\widehat{\rm RGMSE}$ is relatively large for $n=5000$, the very small value of $\det{(\hat{\Sigma}_{MM})}$ for $n=5000$ indicates that the estimate via the modified moments estimation \chris{still has} reasonable performance as the initial value \chris{for} maximum likelihood estimation.
Therefore, modified moments estimation is useful to obtain the maximum likelihood estimates efficiently for a large sample size as well as small and medium sample sizes.
%Therefore, the the goodness of the modified moments estimation as a estimator cannot discuss by only the value of $\widehat{\rm{RGMSE}}$.
% n=5000とかでMMが意味ないわけではなく，初期値に使えるよねって話をする
%一方，MMはそれ単体で最終的な推定量とするのではなく，MLの初期値としていい値を提供するものとしての側面が強いと考えております．その際，両者ともに一致推定量であるためMLの初期値としての機能はある程度担保されるため，RGMSEの値でMMの推定量としての良し悪しは直接語れないのではないかなと思っております．

\kotar{It is noted that the degree of decline of $\det{(\hat{\Sigma})}$ with respect to sample size depends on the estimation method.
Therefore, for $n=500$, the value of $\widehat{\rm{RGMSE}}$ is slightly smaller than for $n=100$.
The tendency for $\widehat{\rm{RGMSE}}$ to not increase monotonically with respect to $n$ is also observed in the unimodal Kato--Jones distribution \citep[Supplementary Material]{kat15}.}

\quad

==> files/6_Application.tex <==
\section{Application} \label{sec:application}

\subsection{Application of modified method of moments estimation}
The proposed \katot{inferential methods are} applied to \katot{the traffic count data of interest}.
The number of samples is 1,121,262, as \chris{mentioned} in Section \ref{data}.
\kota{In this section,} the number of components is fixed to two because two \chris{main} peaks are recognized in the histogram (see Section \katot{6.2 for results for} other numbers of components).
The conditions of the modified method of moments estimation \chris{are} the same \chriss{as} \chris{in} the previous section.
\kotar{Note that \cite{nag23} in Japanese traffic engineering journal also analyzed traffic count data by applying the method proposed in the preprint version of this paper \citep{nag22}.
However, \cite{nag23} only discussed the ultimate results from the viewpoint of traffic engineering and did not discuss theoretical or statistical aspects of the method.
Moreover, they just focused on comparing the results of data from many counters in different locations, whereas this paper interprets the results from a single location in more detail.}

%the comparison between several  location of detction

\begin{figure}[t]
\centering
\includegraphics[clip,keepaspectratio,width=0.75\textwidth]{fig/best.pdf}
\caption{\label{fig:best} \katoss{Plot of the densities of the reparametrized mixture (\ref{eq:kj_mix_density2}) (bold) and \chris{its} components (dashed) estimated via \kota{the modified method of moments estimation.}}}
\end{figure}

\begin{table}
\caption{\label{tab:best} \katoss{\chris{Parameter estimates} associated with the \kota{modified method of moments \katot{estimation}}.}}
\centering
\fbox{
\subtable[Initial value]{
\begin{minipage}{0.45\textwidth}
\begin{center}
\begin{tabular}{*{5}{c}}
$k$ & $\mu_k$ & $\rho_k$ & $\lambda_k$ & $\pi_k'$ \\
\hline
1 & 2.2755 & 0.5322 & 4.9979 & 0.0316 \\
2 & 3.9458 & 0.8131 & 2.0455 & 0.2331 \\
3 & & & & 0.7353 \\
\end{tabular}
\end{center}
\end{minipage}}
\subtable[Estimated parameter]{
\begin{minipage}{0.45\textwidth}
\begin{center}
\begin{tabular}{*{5}{c}}
$k$ & $\katot{\hat{\mu}}_k$ & \katot{$\hat{\rho}_k$} & \katot{$\hat{\lambda}_k$} & \katot{$\hat{\pi}_k'$} \\
\hline
1 & 2.7514 & 0.7322 & 5.3162 & 0.4543 \\
2 & 4.0106 & 0.1947 & 1.1589 & 0.4820 \\
3 & & & & 0.0637 \\
\end{tabular}
\end{center}
\end{minipage}}}
\end{table}

\begin{table}
\caption{\label{tab:bestm} \katot{Values} of the empirical and theoretical trigonometric \katoss{moments} \katot{(t.m.'s)} and \katot{squares of their differences in the best result.}}
\centering
\fbox{
\begin{tabular}{c|cccc}
& & empirical \katot{t.m.} & theoretical \katot{t.m.} & square of \katot{difference} \\
\hline
cosine & $p=1$ & $-3.29\times10^{-1}$ & $-3.29\times10^{-1}$ & $2.95\times10^{-14}$ \\
& $p=2$ & $-7.07\times10^{-2}$ & $-7.07\times10^{-2}$ & $5.64\times10^{-15}$ \\
& $p=3$ & $9.46\times10^{-2}$ & $9.46\times10^{-2}$ & $3.07\times10^{-15}$ \\
& $p=4$ & $-1.61\times10^{-2}$ & $-1.61\times10^{-2}$ & $8.35\times10^{-15}$ \\
\hline
sine &$p=1$ & $-1.23\times10^{-1}$ & $-1.23\times10^{-1}$ & $2.81\times10^{-14}$ \\
& $p=2$ & $-1.18\times10^{-1}$ & $-1.18\times10^{-1}$ & $1.21\times10^{-13}$ \\
& $p=3$ & $1.29\times10^{-2}$ & $1.29\times10^{-2}$ & $4.21\times10^{-16}$ \\
& $p=4$ & $6.97\times10^{-2}$ & $6.97\times10^{-2}$ & $7.43\times10^{-16}$ \\
\end{tabular}}
\end{table}

The optimization is carried out \katot{for} 10,000 initial values.
Fig.\ \ref{fig:best} and Table \ref{tab:best} show the best result \kotar{in the sense that the value of ETM is the smallest} among 10,000 estimations.
\katot{Table \ref{tab:bestm} provides the values of the empirical and theoretical trigonometric moments.
The solid line in Fig.\ \ref{fig:best} represents the estimated density of the mixture and the dashed lines refer to the estimated densities of the components.
\chris{The same convention will be used in} the following figures of fitted densities.}
The value of ETM is $7.06\times10^{-13}$ and that of \chris{the} log-likelihood function is \katos{$-$}1,840,939.
As shown in the right column of Table \ref{tab:bestm}, the difference between the values of empirical and theoretical trigonometric moments \katot{of all the degrees} are approximately 0, which means that \katot{this result} is very close to \katot{the result of ordinary method of moments estimation.}
\cyan{
Nonetheless, we generally need the proposed modified method of moments to ensure that the parameters are within their ranges, as explained in Section 4.2.
Actually, \katot{when the number of components $m$ is set to be greater than two, much larger values of ETM are obtained for some cases and the \katoss{ordinary method of moments} estimates are out of range for some parameters} (see Section \katos{6.2}).}
Also, the \katot{estimated densities} in Fig.\ \ref{fig:best} \chris{fit fairly} \katot{well} to the histogram.
The sharp and negatively skewed peak around $\pi/2$ is represented by the component \katot{with} $k=1$, \katot{while} the gentle peak around $3\pi/2$ is \katot{modelled} by the component \katot{with} $k=2$.

The computation time for 10,000 trials is about \kotar{14} sec.
\kota{The calculation was run on a \katot{Windows 10} computer with \kotar{an Intel Core i9-12900 processor running at 3.20 GHz using 64.0 GB of RAM.}}
Furthermore, about 25\% of 10,000 trials converge to \kotar{almost the same} value \kota{as} the best result.
\kotar{
In this case, 10,000 initial values were used to verify the performance of the modified method of moments estimation.
% 今回は性能を確かめるために10000個もの初期値を用いた
\kotar{The estimates that provide the smallest value of ETM} can be obtained from 25$\%$ of the initial values, which implies that estimation from a much smaller number of initial values (e.g., 100) would be sufficient.
}
% しかし，25%もの初期値から最適な推定量が得られるということは，もっと少ない(e.g. 100)初期値の個数から推定でも最適な推定量が得られることを意味する．
%We confirmed that various initial values reached the estimated parameters close to those in Table \ref{tab:best} \kota{and the initial value in Table \ref{tab:best} is just an example of such initial values.}

\kotar{Note that the modified method of moments estimation is carried out to obtain a good initial value for maximum likelihood estimation, which is more appropriate for such a large sample size, as discussed in Section 5.}

\subsection{Maximum likelihood estimation} \label{sec:mle}
\chris{The} EM algorithm is carried out by setting the initial values as the best estimates from \chris{the} modified method of moments to achieve the maximum likelihood estimation \kotar{efficiently}.
This choice of the initial values seems reasonable because of the large sample size of the data and the consistency of the modified method of moments estimator and maximum likelihood estimator.
\kotar{The conditions of the maximum likelihood estimation \chris{are} the same \chriss{as} \chris{in} the previous section except for the threshold for the termination of the EM algorithm, which is set to 1.}
This threshold is set by the following \chris{reasoning}.
Since the number of samples in this study is more than 1,000,000, the absolute value of \chris{the} log-likelihood function is expected to be \chris{of} that order of magnitude.
Thus, we regard the threshold 1 \chris{as} small enough to \chris{claim} convergence.

\begin{figure}[t]
\centering
\includegraphics[clip,keepaspectratio,width=0.75\textwidth]{fig/EM2.pdf}
\caption{\label{fig:em} \katoss{Plot of the densities of the reparametrized mixture (\ref{eq:kj_mix_density2}) (bold) and \chriss{its} components (dashed) estimated via the EM algorithm.}}
\end{figure}

\begin{table}
\caption{\label{tab:em} \chris{Parameter estimates} associated with the maximum likelihood estimation for the reparametrized mixture (\ref{eq:kj_mix_density2}) via \chris{the} EM algorithm.}
\centering
\fbox{
\begin{tabular}{*{5}{c}}
$k$ & $\hat{\mu}_k$ & $\hat{\rho}_k$ & $\hat{\lambda}_k$ & $\hat{\pi}_k'$ \\
\hline
1 & 2.7572 & 0.7266 & 5.3136 & 0.4536 \\
2 & 4.0107 & 0.1970 & 1.1895 & 0.4825 \\
3 & & & & 0.0639 \\
\end{tabular}}
\end{table}

The result of \chris{the} EM algorithm is shown in Fig.\ \ref{fig:em} and Table \ref{tab:em}.
It takes \chriss{just} two steps to terminate the EM algorithm.
\chris{The} value of ETM \chris{increases along with that of the log-likelihood} during the EM algorithm.
\chris{The} difference \katot{between the parameter estimates} by the modified method of moments and those by the maximum likelihood estimation \katot{is} not \chris{much}.
This implies \chris{that} \kota{the modified method of moments estimate is close to the \kotar{maximum likelihood estimate}, the estimate \chriss{produced} by another consistent estimator.}

\kotar{
In addition, the standard errors for the parameter estimates by the modified method of moments and those by the maximum likelihood estimation are calculated.
The standard errors for the parameter estimates by the modified method of moments are calculated by the nonparametric bootstrap method \citep{dav97}, and those by the maximum likelihood estimation are calculated by the Fisher information matrix for the log-likelihood function due to computation time.}

\begin{table}
\caption{\label{tab:stderr} \kotar{The value of standard errors for the parameter estimates by the modified method of moments and those by the maximum likelihood estimation.}}
\centering
\fbox{
\begin{tabular}{c|ccccc}
 & $k$ & $\hat{\mu}_k$ & $\hat{\rho}_k$ & $\hat{\lambda}_k$ & $\hat{\pi}_k'$ \\
\hline
the modified method of moments & 1 & $5.77\times10^{-2}$ & $2.46\times10^{-2}$ & $1.87\times10^{-1}$ & $8.91\times10^{-3}$\\
& 2 & $5.74\times10^{-2}$ & $2.47\times10^{-2}$ & $1.90\times10^{-1}$ & $5.92\times10^{-3}$\\
& 3 & & & & $6.59\times10^{-2}$\\
\hline
the maximum likelihood estimation & 1 & $6.36\times10^{-3}$ & $3.50\times10^{-3}$ & $2.88\times10^{-2}$ & $3.27\times10^{-3}$\\
& 2 & $6.82\times10^{-3}$ & $1.98\times10^{-3}$ & $9.03\times10^{-3}$ & $3.76\times10^{-3}$\\
& 3 & & & & $3.30\times10^{-3}$\\
\end{tabular}}
\end{table}

\kotar{The results are shown in Table \ref{tab:stderr}.
\katou{These results indicate that,} for all parameters, the values of standard error \katou{of the maximum likelihood estimates} are smaller than those of \katou{the modified method of moments estimates.
However the modified method of moments estimates generally exhibit satisfactory performance, supporting our idea of using these estimates as the initial values of the EM algorithm.
For both the modified method of moments and maximum likelihood estimates, the values of the standard errors of $\hat{\lambda}_k$ are greater than those of the other parameters.}
The values of standard error for the parameter estimates by the maximum likelihood estimation are in between the order of the second and third power of 10, and those by the modified method of moments are in between the order of the one and third power of 10.
%(事実を書いたのですが，ここからどういうことが言えるかがわからなくて考察に困っております，「ETMによる推定値はMLEよりもreliabilityに欠けるが，絶対的な評価では大きな問題はない」といったことを書けばいいのでしょうか？あと，そもそもこの話をどこに挿入するかも迷っております．)\katou{【加藤：「ETMによる推定値はMLEよりもreliabilityに欠けるが，絶対的な評価では大きな問題はない」と書くので良いと思います．そのような旨の考察の例を付け足してみました．場所はここで良いと思います．】}
}



As for the computation time, it takes \kotar{93} sec. for \chris{the} EM algorithm although only two M-steps are conducted in the calculation.
\kota{The calculation environment is the same as that of the previous \katoss{subsection}.}
Compared to the modified method of moments that takes only about \kotar{14} sec. for 10,000 trials, \chris{the} EM algorithm requires \chris{a} longer time.
Therefore, setting the initial value close to the maximum likelihood estimator is necessary to achieve the maximum likelihood estimation by \chris{the} EM algorithm in a feasible computation time.
The proposed modified method of moments is one possible solution for this purpose.

\kotar{Although two parameter estimation methods are introduced in this paper, the maximum likelihood estimation is preferred in terms of the mean squared error of the estimators and usage for model comparison.
The modified method of moments is useful to obtain a good initial value for the maximum likelihood estimation with a short computation time for large sample sizes.}

\begin{figure}[t]
    \begin{center}
			\includegraphics[clip, keepaspectratio, width=0.75\hsize]{fig/last.pdf}
    \end{center}
\caption{\label{fig:rest} \katoss{Plot of the estimated densities of the recovered mixture (\ref{eq:kj_mix_density}) (bold) and their components (dashed).}}
\end{figure}

\begin{table}
\caption{\label{tab:rest} \kotan{\katot{Maximum likelihood estimates \chris{for} the mixture with the recovered original parametrization (\ref{eq:kj_mix_density}).}}}
\centering
\fbox{
\begin{tabular}{*{6}{c}}
$k$ & $\hat{\mu}_k$ & $\hat{\gamma}_k$ & $\hat{\rho}_k$ & $\hat{\lambda}_k$ & $\hat{\pi}_k$ \\
\hline
1 & 2.7572 & 0.3751 & 0.7267 & 5.3136 & 0.4845 \\
2 & 4.0107 & 0.4855 & 0.1970 & 1.1895 & 0.5155 \\
\end{tabular}}
\end{table}

\kota{
Here, the parameters are estimated in the form of the mixture of two Kato--Jones distributions and the uniform distribution (Table \ref{tab:em}(b) and equation (4)).
Actually, we can regard this mixture of three components as the estimated \katot{model}.
Nonetheless, we are also able to reparameterize and recover the estimates of \katot{the} original parameters \katot{(\ref{eq:kj_mix_density})} as discussed in Section 4.1.
As we initially aim to estimate the mixture of two components, we employ the \chriss{latter} in the following.}
% Note that the model with uniform distribution (Table \ref{tab:emm}(b)) is one of the choices.
% It can be reparameterized and interpreted as well.
% In this study, the recovered model is employed from the viewpoint of interpretability.
The \katot{maximum likelihood estimates \chris{obtained via the} EM algorithm} (Fig.\ \ref{fig:em} and Table \ref{tab:em}) are recovered \katot{to} \katot{$\hat{\mu}_k, \hat{\gamma}_k, \hat{\rho}_k, \hat{\lambda}_k$ and ${\hat{\pi}}_k$} \kotann{as shown in Fig.\ \ref{fig:rest} and Table \ref{tab:rest}}.
The \katot{shapes of the two estimated components with $k=1,2$ in Table \ref{tab:em}  slightly change} by adding the restored uniform \katot{component with $k=3$.}

\kotar{In addition, $\hat{\mu}_k, \hat{\gamma}_k, \hat{\rho}_k, \hat{\lambda}_k$ are reparameterized into $\hat{\mu}_k, \hat{\gamma}_k, \hat{\bar{\alpha}}_{2k}, \hat{\bar{\beta}}_{2k}$ for interpretation because
$\hat{\bar{\alpha}}_{2k}$ and $\hat{\bar{\beta}}_{2k}$ can be interpreted as the circular skewness and kurtosis of \citet{bat} as mentioned in Section 3.2.}
The recovered parameters are reparameterized as shown in Table \ref{tab:repa}.
\kotar{The discussion of the parameter values to follow is carried out only for the parameters in Table \ref{tab:repa} because of the interpretability for $\hat{\bar{\alpha}}_{2k}$ and $\hat{\bar{\beta}}_{2k}$.}

\begin{table}
\caption{\label{tab:repa} \kotan{\katot{Maximum likelihood estimates \chris{for} the reparametrized mixture (\ref{eq:repa_density}).}}}
\centering
\fbox{
\begin{tabular}{*{6}{c}}
$k$ & $\hat{\mu}_k$ & $\hat{\gamma}_k$ & $\hat{\bar{\alpha}}_{2k}$ & $\hat{\bar{\beta}}_{2k}$ & $\hat{\pi}_k$ \\
\hline
1 & 2.7572 & 0.3751 & 0.1542 & -0.2248 & 0.4845 \\
2 & 4.0107 & 0.4855 & 0.0356 & 0.0888 & 0.5155 \\
\end{tabular}}
\end{table}

\subsection{\kota{Discussion}}

Here, we discuss the interpretation of the estimated models with the recovered parametrizations (\ref{eq:repa_density}) given in Table \ref{tab:repa}.
As shown in Fig.\ \ref{fig:rest}, the densities of the mixture fit fairly well to the histogram for the entire day, such as the sharp peak in the morning and the gentle peak in the evening.
The numerically calculated morning mode and evening mode of \kotar{the whole distribution of }the mixture are 7:32 and 15:56, respectively.

The two components divide the mixture into 48.5$\%$ and 51.5$\%$ as denoted by each value of $\pi_k$.
Each peak roughly represents the morning and evening traffic.
The peak of the component with $k=1$ is sharp and negatively skewed.
Its mean, $\hat{\mu}_1$, is around 10:32, and its mode is around 7:28 \citep[Supplementary Material]{kat15}.
The mode of the component with $k=1$ is close to the morning mode of the mixture because the component with $k=1$ is dominant around the morning.
The shape is characterized by large $\hat{\bar{\alpha}}_{21}$ and negatively large $\hat{\bar{\beta}}_{21}$.
On the other hand, the peak of the component with $k=2$ is gentle and positively skewed.
Its mean, $\hat{\mu}_2$, is around 15:19, and its mode is around 16:37.
The mode of the component with $k=2$ and the evening mode of the mixture are apart because the tail of the component with $k=1$ is contained even in the evening part of the mixture.
The shape is characterized by small $\hat{\bar{\alpha}}_{22}$ and positively small $\hat{\bar{\beta}}_{22}$.

The peak period of the component with $k=1$ is from 7:00 to 8:00, and its shape is remarkably sharp and quick-rising, which is described by large $\hat{\bar{\alpha}}_{21}$ and negatively large $\hat{\bar{\beta}}_{21}$.
This is explained by the actual situation that many drivers would like to arrive in central Osaka around the same time, like 8:30 and 9:00, which is the typical start time for working in Japan.
On the other hand, the peak period of the component with $k=2$ is from 15:00 to 19:00, and its shape is gradual and positively skewed, which is described by small $\hat{\bar{\alpha}}_{22}$ and positively small $\hat{\bar{\beta}}_{22}$.
This may be because drivers do not have to leave their office at the same time, which is different from morning hours.
Some of them may decide to make their departure time earlier or later than peak hour to avoid traffic congestion.
In addition, the positively skewed shape may imply that they also avoid returning home too late.

These interpretations are made by focusing on the shape around the mode of each peak.
It is more difficult to understand the traffic flow volume around the tails of both components.
For example, the first component still has a moderate probability at around 16:00, which cannot be included in the morning rush hour.
One possible explanation is that the first component represents the outward trip, including morning commuting, commercial vehicles, etc.
For example, many commercial vehicles travel from Kobe to Osaka during the daytime.
In addition, some people make their first trip in the evening because they work at night or go shopping.
People who work at night are more likely to use their vehicles for commuting than those who work in the daytime, as public transport does not operate after midnight.
This could explain the first component having a larger probability than the second component after around 22:00.
Similarly, the second component represents the day's return trips, including evening commuting.
As round and migration trips during the daytime, for example, may be included in the second component, it already has a moderate value even in the morning hours.
Note that outward and return trips are observed only once because all recorded traffics are in the same direction.

Finally, we compare our results with some phenomena typically mentioned in the traffic engineering field.
First, the difference in the value of $\hat{\bar{\alpha}}_{2}$ between the two components is consistent with the concept of departure time choice in traffic engineering \citep{nol95}.
In general, drivers choose their departure time by estimating backward from the time they want to arrive.
\cite{ale15} indicate that many drivers depart within short periods in the morning (i.e., traffic is concentrated), while drivers depart within longer periods in the evening and later.
Second, 30$\%$ of Hanshin Expressway users are for commercial purposes \citep[(in Japanese)]{han}.
Assuming that people make outward commercial trips after they start working, the tail of the first components around noon is likely to contain commercial vehicles at a certain level.
Therefore, the interpretation mentioned above that the first component is for the outward trips of the day and the second one is for the return trips is reasonable to some extent.
Note that the share of large vehicles on this road is 13.6$\%$ in total and less than 30$\%$ even in the midnight period, although one might expect that the freight traffic is the main component after midnight (see Appendix B Supplementary Material).
Therefore, no peak for freight traffic in the midnight period is found in the histograms, nor are such peaks found in the estimated model.
Since these discussions are only derived from traffic volume data, it is necessary to further develop the interpretations by combining trip purpose data and origin and destination data.
Nonetheless, it would be a contribution of this paper that the proposed model that only uses traffic volume information is consistent with various concepts used in traffic engineering.

% %「出勤に代表されるような最初のトリップ」「帰宅に代表されるような2個め以降のトリップ」,二個目以降＝2個めが帰宅じゃない場合は早く立ち上がる？？？
% \katot{Here we discuss the interpretation of the estimated models with the recovered parametrizations (\ref{eq:repa_density}) given in Table \ref{tab:repa}.} %There are two components \katot{with $k=1$ and $2$} after the recovery.
% \kotar{Once again, note that vehicles commuting to their office and returning home are observed only once in the morning or evening.}
% \katot{As} $\hat{\pi}_1$ and $\hat{\pi}_2$ have similar values, the \katot{weights} of these components \katot{are} approximately the same. 
% Next, the \katot{peak of the component with $k=1$} is sharp and negatively skewed.
% Its mean, $\hat{\mu}_1$, is around 10:32 and its mode is around 7:28
% \cyan{\citep[Supplementary Material]{kat15}}.
% The shape is characterized by large $\hat{\bar{\alpha}}_{21}$ and negatively large $\hat{\bar{\beta}}_{21}$.
% As explained in Section \ref{data}, this result is consistent with the actual situation that many drivers would like to arrive in central Osaka \chris{at} just around the same time like 8:30 and 9:00.
% On the other hand, the \katot{peak of the component with $k=2$} is gentle and positively skewed.
% Its mean, $\hat{\mu}_2$, is around 15:19 and its mode is around 16:37.
% The shape is characterized by small $\hat{\bar{\alpha}}_{22}$ and positively small $\hat{\bar{\beta}}_{22}$.
% The result shows that evening traffic flow does not concentrate in a short time compared with \chris{the} morning one.
% This may be because drivers do not have to leave their office at the same \chris{time}, which is different from morning hours.
% Perhaps, some of them decide \chris{to make} their departure time earlier or later than peak hour to avoid traffic congestion.
% In addition, the positively skewed shape may imply that they also avoid \chris{being} too late returning home.

% These interpretations are made by focusing on the shape around the mode of each peak.
% \chris{It} is \katos{more} difficult to understand the traffic flow volume around the tails of both components.
% For example, the first component still has a moderate probability at around 16:00, which cannot be included in the morning rush hour.
% One possible explanation is that the first component represents the first trip of the day that includes the morning commuting.
% While \chriss{others} make their first trip in the evening because they work at nighttime or they go shopping.
% \cyan{Especially, people \katos{who} work at night are more likely to use their own vehicles for commuting than \katos{those} who work in the daytime as public transport is not operating \chris{after} midnight.
% This could be an explanation \chris{for} the first component \chris{having} larger probability than the second component after around 22:00.
% }
% Similarly, the second component represents the second and subsequent trips of the day that include the evening commuting.
% As round \cyan{and migration} trips during daytime, for example, may be included in the second component, it already has a moderate value even in the morning hours.
% Nonetheless, further investigation is necessary for more \chris{detailed} analyses, e.g., considering the effect of commercial trips and heavy vehicles by changing the number of components.% 公共交通，夜は車で出勤しがち，運送業の貨物車などがある，などなど

==> files/7_Othermodel.tex <==
\section{Comparison with other models} \label{sec:comparison}

\subsection{Mixtures of \kotar{other distributions}} \label{sec:comparison_other}

\kotar{We compare other \kota{multimodal} distributions with our proposed model in terms of \katot{practicability and fit}.
The distributions considered here are the mixture of von Mises distributions (MovM), the mixture of wrapped Cauchy distributions (MowC), the mixture of sine-skewed von Mises distributions (MossvM) and the mixture of sine-skewed wrapped Cauchy distributions (MosswC) whose densities are given by}
\begin{eqnarray*}
f_{MovM}(\theta) &=&  \sum_{k=1}^m \frac{\pi_k}{2\pi I_{0}(\kappa_k)} \exp(\kappa_{k}\cos(\theta-\mu_k)),\\
f_{MowC}(\theta) &=&  \sum_{k=1}^m \frac{\pi_k}{2\pi} \frac{1-\rho_k^2}{1+\rho_k^2-2\rho_k\cos{(\theta-\mu_k)}},\\
f_{MossvM}(\theta) &=&  \sum_{k=1}^m \frac{\pi_k(1+\lambda_k\sin(\theta-\mu_k))}{2\pi I_{0}(\kappa_k)} \exp(\kappa_{k}\cos(\theta-\mu_k)),\\
f_{MosswC}(\theta) &=&  \sum_{k=1}^m \frac{\pi_k}{2\pi} \frac{1-\rho_k^2}{1+\rho_k^2-2\rho_k\cos{(\theta-\mu_k)}}(1+\lambda_k\sin(\theta-\mu_k)),\\
\end{eqnarray*}
respectively, where $\mu_k \in [0, 2\pi)$ is the mean direction, \kotar{$\kappa_k \in [0, \infty)$ and $\rho_k \in [0, 1]$ are concentration parameters, $\lambda_k \in [-1, 1]$ is a skewing parameter}, $I_{0}(\cdot)$ is the modified Bessel function of the first kind and order zero\chris{,} $m \in \mathbb{N}$ is the number of components of the mixture and $0 < \pi_1,\ldots,\pi_m < 1$ are the weights of the components satisfying $\sum_{k=1}^m \pi_k =1 $.
\kotar{The number of free parameters for MovM and MowC is $3m-1$, and that for MossvM and MosswC is $4m-1$.
These distributions are popular mixtures discussed, e.g., in \citet{wal00,moo03,ban05,mul20,miy20}.
Note that the mixture of sine-skewed wrapped Cauchy is a submodel of the proposed model \cite[Supplementary Material]{kat15}.}

\kotar{The 50-fold cross-validation is conducted to compare the performance of the proposed model with that of these four existing models.
The cross-validated log-likelihood is employed as the criterion for comparison \citep{smy00}.
The number of components is set to two, as in our proposed model.}

\begin{table}
\caption{\label{tab:cross1} \kotar{The average value of cross-validated log-likelihood function in 50-fold cross validation for MovM, MowC, MossvM, MosswC and proposed model.}}
\centering
\fbox{
\begin{tabular}{*{4}{c}}
model & log-likelihood function\\
\hline
proposed & -36818.5\\
MovM & -37059.4\\
MowC & -37731.7\\
MossvM & -37026.3\\
MosswC & -36855.3\\
\end{tabular}}
\end{table}

\kotar{
Table \ref{tab:cross1} shows each model's average value of the cross-validated log-likelihood function.
The predictive performance of the proposed model is superior to the other models because the value for the proposed model is the largest.
\kotarr{
As an example of a plot of the estimated densities, Fig.~\ref{fig:vm} shows the maximum likelihood fits of the densities of MovM, the most well-known mixture of circular distributions, with two components.
The goodness of fit looks significantly worse than in the proposed model shown in Fig.~\ref{fig:rest}.
Particularly, the distorted peak around $\pi/2$ and the gradual peak around $3\pi/2$ are not represented.}
In contrast to the proposed model that allows varying kurtosis and skewness values, MovM and MowC do not allow both, and MossvM and MosswC do not allow varying kurtosis.
In terms of the number of parameters, MovM and MowC have $m$ fewer than the proposed model, and MossvM and MosswC have the same.
The proposed model is superior to the other models in terms of predictive performance because the proposed model can vary its shape flexibly with a small number of parameters.}
\kotarr{In addition to the cross-validation, a comparison of the proposed model with other models using simulation studies is provided in Appendix C in Supplementary Material.}

\begin{figure}[t]
    \begin{center}
			\includegraphics[clip, keepaspectratio, width=0.75\hsize]{fig/vm.pdf}
    \end{center}
\caption{\label{fig:vm} Plot of maximum likelihood fit of the density of MovM with two components.}
\end{figure}

\subsection{Our \katot{mixture with more than two components}}%m=8くらいまで計算しましたがどうしますか？
%We assume two components in Section 5 because two typical peaks can be recognized in the histogram.
\katot{We estimate} the mixed Kato--Jones distributions \katot{(\ref{eq:repa_density})} whose number of components $m$ \katot{is} more than two.
\kota{In this \katot{subsection}, models \katot{with $m \leq 6$ are discussed} because of stability of estimation; estimation for the model \katot{with  $m > 6$} \chris{was} carried out but the \chris{results were} unstable.}
\chris{Recall} that the histogram shows two peaks that can be interpreted as shown above and the assumption of more than two peaks is not necessarily insightful from the transport engineering viewpoint.
As such, the main purpose \chris{of} this subsection is not to find the most accurate number of components but \chris{to find out} what \chris{shapes} of distributions will be \chris{obtained}.
%However, there are not only two types traffic; morning traffic and evening traffic, but also another kind of traffic such as commercial traffic, long-distance lorry and journey.
%Therefore, other models whose number of components is more than 2 are estimated.

\kotar{The 50-fold cross-validations for the proposed model, whose number of components $m$ is from 2 to 6, are conducted.}
\kotan{The conditions for the estimation are the same as those in Section 5.}

\begin{table}
\caption{\label{tab:cross2} \kotar{The average value of cross-validated log-likelihood function in 50-fold cross validation for proposed model whose number of components $m$ from 2 to 6}}
\centering
\fbox{
\begin{tabular}{*{4}{c}}
$m$ & log-likelihood function\\
\hline
2 & -36818.5\\
3 & -36818.7\\
4 & -36808.6\\
5 & -36817.6\\
6 & -36820.2
\end{tabular}}
\end{table}

\kotar{
Table \ref{tab:cross2} shows the average value of the cross-validated log-likelihood function for each number of components.
The model whose number of components $m=4$ is the best because the value for the proposed model is the largest.
The plot and value of the parameter for the estimated model whose number of components $m=4$ are shown in Fig.\ \ref{fig:m4} and Table \ref{tab:m4}.
Note that the number of bins in Fig.\ \ref{fig:m4} is 96 (i.e., the width of the bin equals 15 minutes) to visualise the small peak around 15:00 described by the component with $k=3$.}

\kotar{
In the results of $m=4$, two prominent components with $k=1, 2$ have a large value of $\hat{\pi}_k$.
As well as the results of $m=2$, the components with $k=1,2$ represent the peak around $\pi/2$ and $3\pi/2$, respectively.
However, the component with $k=2$ for $m=4$ is not skewed compared to the component with $k=2$ for $m=2$ shown in Fig.\ \ref{fig:rest}.
Not only the component with $k=2$ but also that with $k=4$ in the results of $m=4$ represent the shape between $3\pi/2$ and $2\pi$ that is represented by only one component with $k=2$ in the results of $m=2$.
In addition, the component \katot{with $k=3$} has \chris{a} small value of \katot{$\hat{\pi}_3$} and represents the small peak around 16:00 seen in the histogram.}

\kotar{
The components with $k=3,4$ may not be meaningful from the transport engineering viewpoint;
they only represent the trivial peak along \chris{with} the improvement of the value of \chris{the} log-likelihood function.
The interpretation of the parameters for these smaller components is difficult with only the traffic volume data.
Some additional information, such as each vehicle's origin, destination, and trip purpose, may help the interpretation of the parameters.}
%Further consideration of determining the appropriate number of components may be necessary.
%The values of AIC and BIC suggest a larger number of components.
%The small components seen in these cases might be generated by some unknown factors and phenomena.
%Nonetheless, from the viewpoints of interpretability of the result and feasibility of the calculation, we regard $m=2$ as the most reasonable numbers of components in this study.

\begin{figure}[t]
    \begin{center}
			\includegraphics[clip, keepaspectratio, width=0.75\hsize]{fig/m4.pdf}
    \end{center}
\caption{\label{fig:m4} \katoss{Plot of maximum likelihood fits of the densities with the numbers of components $m=4$.}}
\end{figure}

\begin{table}
\caption{\label{tab:m4} Maximum likelihood estimates of the parameters of Kato--Jones mixtures (\ref{eq:repa_density}) whose numbers of components $m=4$.}
\centering
\fbox{
\begin{tabular}{*{6}{c}}
$k$ & $\hat{\mu}_k$ & $\hat{\gamma}_k$ & $\hat{\bar{\alpha}}_{2k}$ & $\hat{\bar{\beta}}_{2k}$ & $\hat{\pi}_k$ \\
\hline
 1 & 2.6665 & 0.4376 & 0.2128 & -0.2452 & 0.3855 \\
 2 & 3.7380 & 0.5065 & 0.0076 & 0.0225 & 0.4907 \\
 3 & 4.3642 & 0.4887 & 0.3402 & -0.2284 & 0.0285 \\
 4 & 5.2889 & 0.6037 & 0.2628 & -0.2166 & 0.0952 \\
\end{tabular}}
\end{table}

==> files/8_Conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

In this paper, we estimated the probability distribution of the variation of traffic volume within an average weekday.
We employed the mixture of Kato--Jones distributions, which 
%is one of the circular distributions and 
can provide a wide range of skewness and kurtosis \katot{for each component}.
%for the variation of traffic volume within an average weekday with using the raw data of traffic counter.
To estimate the parameters of these distributions, we developed the modified method of moments.
\kota{
This method \chris{ensures} that the estimated parameters 
% One of the advantages of the method is that the estimate 
always belong to the parameter space.
}
\katos{Then the maximum likelihood method for the proposed mixture was established using the EM algorithm}.

The proposed method was applied to \chris{some} traffic counter data \chris{from} Japan. 
% In the result of the number of components $m=2$, 
As a result, the data were classified into two components, which were interpreted as the morning and evening traffic.
%by the proposed method.
Some reasonable explanations for these components are suggested\chris{,} that the difference in \chris{the} shapes \chris{of the components} might be caused by the different \chris{behaviours underlying} the commuting trips between morning and evening hours.
\cyan{In addition, the modified method of moments was \katoss{seen} to allow for fast calculation and provided \chris{a} reasonable initial value \chris{for} maximum likelihood estimation.}
\katos{With this initial value, the EM algorithm provided reasonable maximum likelihood \chris{estimates}.}
% the method works quickly and the estimate from the method is a useful 

% The first distribution is negatively skewed peak whose mode is 7:28.
% This result is consistent with the actual situation that many drivers would like to arrive central Osaka in just around the same time as 8:30 and 9:00.
% On the other hand, the second distribution is gentle and positively skewed peak whose mode is 16:37.
% This result shows that evening traffic does not concentrate compared with morning one.
% This may be because drivers do not have to leave their office at the same timing.
% We estimate the model with another number of components from $m=3$ to $m=8$.
% The value of $AIC$ and $BIC$ get better as $m$ increases.
% On the other hand, the larger $m$ needs the longer computation time.
% Moreover, the interpretation of the all components is difficult.
%From the viewpoints of interpretability of the result and the feasibility of the calculation, we regard that $m=2$ is one of the reasonable number of components in this study.
%According to \katot{information criteria} such as $AIC$ and $BIC$, \chris{a} larger number of components than two resulted in better \chris{estimation}.
\kotar{According to the cross-validated log-likelihood function, the model with the number of components $m=4$ is the best.
However, the interpretation of the trivial components in the model is difficult thus far.
Further consideration of missing factors that generate third and later components may be necessary in future work.
Additional information, such as each vehicle's origin, destination, and trip purpose, would be useful.
In addition, we assume the IID property for all traffic data in the modeling, and we regard this assumption as acceptable, as mentioned in the supplementary Material.
However, modeling the dependent characteristics of the arrival interval, if it exists, is one of the principal and important issues to be dealt with in the future.}


% However, if we have another data such as the data of the origin of each vehicle or the purpose of their trip, the more interpretation of another number of components can be improved.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
